Sesqui-Pushout Rewriting: Concurrency, Associativity and Rule Algebra Framework

Sesqui-pushout (SqPO) rewriting is a variant of transformations of graph-like and other types of structures that fit into the framework of adhesive categories where deletion in unknown context may be implemented. We provide the first account of a concurrency theorem for this important type of rewriting, and we demonstrate the additional mathematical property of a form of associativity for these theories. Associativity may then be exploited to construct so-called rule algebras (of SqPO type), based upon which in particular a universal framework of continuous-time Markov chains for stochastic SqPO rewriting systems may be realized.

==> eptcsdata.tex <==
\providecommand{\firstpage}{23}
\providecommand{\publicationstatus}{Rachid Echahed and Detlef Plump (Eds.): Tenth International\\ Workshop on Graph Computation Models (GCM 2019)\\
EPTCS 309, 2019, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.309.2}{10.4204/EPTCS.309.2}}
\pdfoutput=1

